Assessing Translation capabilities of Large Language Models involving English and Indian Languages

Generative Large Language Models (LLMs) have achieved remarkable advancements in various NLP tasks. In this work, our aim is to explore the multilingual capabilities of large language models by using machine translation as a task involving English and 22 Indian languages. We first investigate the translation capabilities of raw large language models, followed by exploring the in-context learning capabilities of the same raw models. We fine-tune these large language models using parameter efficient fine-tuning methods such as LoRA and additionally with full fine-tuning. Through our study, we have identified the best performing large language model for the translation task involving LLMs, which is based on LLaMA. Our results demonstrate significant progress, with average BLEU scores of 13.42, 15.93, 12.13, 12.30, and 12.07, as well as CHRF scores of 43.98, 46.99, 42.55, 42.42, and 45.39, respectively, using 2-stage fine-tuned LLaMA-13b for English to Indian languages on IN22 (conversational), IN22 (general), flores200-dev, flores200-devtest, and newstest2019 testsets. Similarly, for Indian languages to English, we achieved average BLEU scores of 14.03, 16.65, 16.17, 15.35 and 12.55 along with chrF scores of 36.71, 40.44, 40.26, 39.51, and 36.20, respectively, using fine-tuned LLaMA-13b on IN22 (conversational), IN22 (general), flores200-dev, flores200-devtest, and newstest2019 testsets. Overall, our findings highlight the potential and strength of large language models for machine translation capabilities, including for languages that are currently underrepresented in LLMs.

==> Average-co-relation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrr}
\textbf{English to INs} & \multicolumn{3}{r}{\textbf{Average Across Languages}} \\
\textbf{Co-relation scores} & \textbf{S} & \textbf{P} & \textbf{K} \\
\textbf{COMET} & 0.4568 & 0.5236 & 0.32042
\textbf{Llama-2-7b-Adpt} & 0.45322 & 0.52096 & 0.3371 \\
\textbf{Llama-2-13b-Adpt} & \textbf{0.4574} & \textbf{0.53744} & \textbf{0.3437} \\
\textbf{Mistral-7b-Adpt} & 0.44538 & 0.50744 & 0.33622 \\
\textbf{Llama-2-7b-Adpt-Full} & 0.43678 & 0.4945 & 0.33852 \\
\textbf{Llama-2-13b-Adpt-Full} & 0.36608 & 0.32434 & 0.28216 \\
\textbf{Llama-2-7b-Adpt-Trans} & 0.39814 & 0.4643 & 0.2972 \\
\textbf{Llama-2-13b-Adpt-Trans} & 0.4429 & 0.50322 & 0.33116 \\
\textbf{Mistral-7b-Adpt-Trans} & 0.41762 & 0.47528 & 0.31674 \\
\end{tabular}%
}
\end{table}

==> langs-v0.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[h]
\centering
\resizebox{2.05\columnwidth}{!}{%
\begin{tabular}{lcccccccccccccll|ccll|cc|c}
\toprule
\textbf{Language Family} & \multicolumn{15}{c|}{{\ul \textbf{Indo-Aryan}}}                                                                                                                                                                                                                                  & \multicolumn{4}{c|}{{\ul \textbf{Dravidian}}}                                                               & \multicolumn{2}{c|}{{\ul \textbf{Sino-Tibetan}}} & {\ul \textbf{Austroasiatic}} \\
\textbf{Language}        & \textbf{asm} & \textbf{ban} & \textbf{kas} & \textbf{snd} & \textbf{urd} & \textbf{doi} & \textbf{hin} & \textbf{gom} & \textbf{mai} & \textbf{mar} & \textbf{nep} & \textbf{san} & \textbf{guj} & \multicolumn{1}{c}{\textbf{odi}} & \multicolumn{1}{c|}{\textbf{pan}} & \textbf{kan} & \textbf{mal} & \multicolumn{1}{c}{\textbf{tam}} & \multicolumn{1}{c|}{\textbf{tel}} & \textbf{mni}  & \textbf{brx}            & \textbf{sat}        \\
\cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-13}\cmidrule(lr){14-14}\cmidrule(lr){15-15}\cmidrule(lr){16-16}\cmidrule(lr){17-20}\cmidrule(lr){21-22}\cmidrule(lr){23-23}
\textbf{Language Script} & \multicolumn{2}{c}{Bangla}  & \multicolumn{3}{c}{Perso-Arbic}            & \multicolumn{7}{c}{Devanagari}                                                                         & Gujarati     & Odia                             & Gurumukhi                         & Kannada      & Malayalam    & Tamil                            & Telugu                            & Meitei        & Devanagari              & Ol Chik             \\ 
\textbf{No of Letters}   & \multicolumn{2}{c}{50}      & \multicolumn{3}{c}{32}                     & \multicolumn{7}{c}{48}                                                                                 & 48           & \multicolumn{1}{c}{52}                               & \multicolumn{1}{c|}{45}                                & \multicolumn{1}{c}{49}           & \multicolumn{1}{c}{56}           & \multicolumn{1}{c}{31}                               & \multicolumn{1}{c|}{56}                                & 27            & \multicolumn{1}{c|}{48} & 30                  \\ 
\hdashline
\textbf{Models (Vocab)}   &&&&&&&&&&&&&&&&&&&&&& \\
\hdashline

\textbf{BLOOM (250680)}   & \multicolumn{2}{c}{(48,02)}      & \multicolumn{3}{c}{(20,12)}                     & \multicolumn{7}{c}{(46,02)}                                                                                 & (40,08)           & \multicolumn{1}{c}{(46,06)}                               & \multicolumn{1}{c|}{(43,02)}                                & \multicolumn{1}{c}{(49,00)}           & \multicolumn{1}{c}{(53,03)}           & \multicolumn{1}{c}{(30,01)}                               & \multicolumn{1}{c|}{(52,04)}                                & (00,27)            & \multicolumn{1}{c|}{(46,02)} & (00,30)                  \\

\textbf{FALCON (65024)}   & \multicolumn{2}{c}{(00,50)}      & \multicolumn{3}{c}{(12,20)}                     & \multicolumn{7}{c}{(02,46)}                                                                                 & (00,48)           & \multicolumn{1}{c}{(00,48)}                               & \multicolumn{1}{c|}{(00,45)}                                & \multicolumn{1}{c}{(00,49)}           & \multicolumn{1}{c}{(00,56)}           & \multicolumn{1}{c}{(00,31)}                               & \multicolumn{1}{c|}{(52,04)}                                & (00,27)            & \multicolumn{1}{c|}{(02,46)} & (00,30)                  \\
\textbf{LLAMA-1,2 (32024)}   & \multicolumn{2}{c}{(10,40)}      & \multicolumn{3}{c}{(11,21)}                     & \multicolumn{7}{c}{(17,31)}                                                                                 & (01,47)           & \multicolumn{1}{c}{(00,52)}                               & \multicolumn{1}{c|}{(04,41)}                                & \multicolumn{1}{c}{(02,47)}           & \multicolumn{1}{c}{(33,23)}           & \multicolumn{1}{c}{(19,12)}                               & \multicolumn{1}{c|}{(01,55)}                                & (00,27)            & \multicolumn{1}{c|}{(17,31)} & (00,30)                  \\
\textbf{MISTRAL (32052)}   & \multicolumn{2}{c}{(22,28)}      & \multicolumn{3}{c}{(18,14)}                     & \multicolumn{7}{c}{(22,26)}                                                                                 & (05,43)           & \multicolumn{1}{c}{(00,52)}                               & \multicolumn{1}{c|}{(43,02)}                                & \multicolumn{1}{c}{(31,18)}           & \multicolumn{1}{c}{(52,04)}           & \multicolumn{1}{c}{(08,22)}                               & \multicolumn{1}{c|}{(11,45)}                                & (00,27)            & \multicolumn{1}{c|}{(22,26)} & (00,30)                  \\
\textbf{MPT (50277)}   & \multicolumn{2}{c}{(05,45)}      & \multicolumn{3}{c}{(11,21)}                     & \multicolumn{7}{c}{(27,21)}                                                                                 & (02,46)           & \multicolumn{1}{c}{(00,52)}                               & \multicolumn{1}{c|}{(00,45)}                                & \multicolumn{1}{c}{(00,49)}           & \multicolumn{1}{c}{(01,55)}           & \multicolumn{1}{c}{(05,26)}                               & \multicolumn{1}{c|}{(03,53)}                                & (00,27)            & \multicolumn{1}{c|}{(27,21)} & (00,30)                  \\
\textbf{OPT (50265)}   & \multicolumn{2}{c}{(00,50)}      & \multicolumn{3}{c}{(11,21)}                     & \multicolumn{7}{c}{(01,47)}                                                                                 & (00,48)           & \multicolumn{1}{c}{(00,52)}                               & \multicolumn{1}{c|}{(00,45)}                                & \multicolumn{1}{c}{(00,49)}           & \multicolumn{1}{c}{(00,56)}           & \multicolumn{1}{c}{(00,31)}                               & \multicolumn{1}{c|}{(00,56)}                                & (00,27)            & \multicolumn{1}{c|}{(01,47)} & (00,30)                  \\
\bottomrule
\end{tabular}%
}
\caption{The language support of various LLMs for 22 Indian languages, along with the corresponding families, scripts, and letters representing each language. In each tuple (xx, yy), the first value represents the number of language-specific characters, while the second value indicates the count of byte-supported characters in respective LLM and for respective language.}
\label{tab:llms_details}
\end{table*}

==> llms_lang_support.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering\small
\setlength{\tabcolsep}{1ex}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllllllllllllllllllll}
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{Vocab size} & \multicolumn{2}{c}{\textbf{Bangla script}} & \multicolumn{3}{c}{\textbf{Perso-Arbic script}} & \multicolumn{8}{c}{\textbf{Devanagari}} & \multicolumn{10}{c}{\textbf{Language specific script}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-7}\cmidrule(lr){5-7}\cmidrule(lr){8-15}\cmidrule(lr){16-25}
 &  & \multicolumn{1}{c}{asm} & \multicolumn{1}{c}{ban} & \multicolumn{1}{c}{kas} & \multicolumn{1}{c}{snd} & \multicolumn{1}{c}{urd} & \multicolumn{1}{c}{brx} & \multicolumn{1}{c}{doi} & \multicolumn{1}{c}{hin} & \multicolumn{1}{c}{gom} & \multicolumn{1}{c}{mai} & \multicolumn{1}{c}{mar} & \multicolumn{1}{c}{nep} & \multicolumn{1}{c}{san} & \multicolumn{1}{c}{guj} & \multicolumn{1}{c}{kan} & \multicolumn{1}{c}{mal} & \multicolumn{1}{c}{mni} & \multicolumn{1}{c}{odi} & \multicolumn{1}{c}{pan} & \multicolumn{1}{c}{sat} & \multicolumn{1}{c}{tam} & \multicolumn{1}{c}{tel} & eng \\ \midrule 
\textit{\textbf{BLOOM}} & 250680 & \multicolumn{1}{l}{(48, 2)} & \multicolumn{1}{l}{(48, 2)} & \multicolumn{1}{l}{(49, 12)} & \multicolumn{1}{l}{(48, 19)} & \multicolumn{1}{l}{(48, 3)} & \multicolumn{1}{l}{(58, 0)} & \multicolumn{1}{l}{(59, 1)} & \multicolumn{1}{l}{(67, 2)} & \multicolumn{1}{l}{(66, 2)} & \multicolumn{1}{l}{(67, 3)} & \multicolumn{1}{l}{(65, 1)} & \multicolumn{1}{l}{(63, 1)} & \multicolumn{1}{l}{(65, 2)} & \multicolumn{1}{l}{(57, 8)} & \multicolumn{1}{l}{(62, 0)} & \multicolumn{1}{l}{(66, 3)} & \multicolumn{1}{l}{(0, 44)} & \multicolumn{1}{l}{(56, 6)} & \multicolumn{1}{l}{(55, 2)} & \multicolumn{1}{l}{(0, 43)} & \multicolumn{1}{l}{(46, 1)} & \multicolumn{1}{l}{(61, 4)} & 127581 \\ 
\textit{\textbf{FACLON}} & 65024 & \multicolumn{1}{l}{(0, 61)} & \multicolumn{1}{l}{(0, 61)} & \multicolumn{1}{l}{(12, 49)} & \multicolumn{1}{l}{(15, 52)} & \multicolumn{1}{l}{(12, 39)} & \multicolumn{1}{l}{(2, 56)} & \multicolumn{1}{l}{(2, 58)} & \multicolumn{1}{l}{(2, 67)} & \multicolumn{1}{l}{(2, 66)} & \multicolumn{1}{l}{(2, 68)} & \multicolumn{1}{l}{(2, 64)} & \multicolumn{1}{l}{ (2, 62)} & \multicolumn{1}{l}{(2, 65)} & \multicolumn{1}{l}{(0, 65)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(0, 69)} & \multicolumn{1}{l}{(0, 44)} & \multicolumn{1}{l}{(0,62)} & \multicolumn{1}{l}{(0, 57)} & \multicolumn{1}{l}{(0, 43)} & \multicolumn{1}{l}{(0, 47)} & \multicolumn{1}{l}{(0, 65)} & 62278 \\ 
\textit{\textbf{LLAMA-1,2}} & 32024 & \multicolumn{1}{l}{(23, 38)} & \multicolumn{1}{l}{(24, 37)} & \multicolumn{1}{l}{(40, 21)} & \multicolumn{1}{l}{(45, 22)} & \multicolumn{1}{l}{(38, 13)} & \multicolumn{1}{l}{(38, 20)} & \multicolumn{1}{l}{(38, 22)} & \multicolumn{1}{l}{(38, 31)} & \multicolumn{1}{l}{(38, 30)} & \multicolumn{1}{l}{(38, 32)} & \multicolumn{1}{l}{(38, 28)} & \multicolumn{1}{l}{(38, 26)} & \multicolumn{1}{l}{(38, 29)} & \multicolumn{1}{l}{(1, 64)} & \multicolumn{1}{l}{(2, 60)} & \multicolumn{1}{l}{(33, 36)} & \multicolumn{1}{l}{(0, 44)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(4, 53)} & \multicolumn{1}{l}{(0, 43)} & \multicolumn{1}{l}{(19, 28)} & \multicolumn{1}{l}{(1, 64)} & 27007 \\ 
\textit{\textbf{MISTRAL}} & 32052 & \multicolumn{1}{l}{(33, 28)} & \multicolumn{1}{l}{(34, 27)} & \multicolumn{1}{l}{(47, 14)} & \multicolumn{1}{l}{(47, 20)} & \multicolumn{1}{l}{(45, 6)} & \multicolumn{1}{l}{(43, 15)} & \multicolumn{1}{l}{(43, 17)} & \multicolumn{1}{l}{(43, 26)} & \multicolumn{1}{l}{(43, 25)} & \multicolumn{1}{l}{(43, 27)} & \multicolumn{1}{l}{(43, 23)} & \multicolumn{1}{l}{(43, 21)} & \multicolumn{1}{l}{(43, 24)} & \multicolumn{1}{l}{(5, 60)} & \multicolumn{1}{l}{(18, 44)} & \multicolumn{1}{l}{(4, 65)} & \multicolumn{1}{l}{(0, 44)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(2, 55)} & \multicolumn{1}{l}{(0, 43)} & \multicolumn{1}{l}{(22, 25)} & \multicolumn{1}{l}{(11, 54)} & 27077 \\ 
\textit{\textbf{MPT}} & 50277 & \multicolumn{1}{l}{(5, 56)} & \multicolumn{1}{l}{(5, 56)} & \multicolumn{1}{l}{(31, 30)} & \multicolumn{1}{l}{(35, 32)} & \multicolumn{1}{l}{(30, 21)} & \multicolumn{1}{l}{(22, 36)} & \multicolumn{1}{l}{(22, 38)} & \multicolumn{1}{l}{(22, 47)} & \multicolumn{1}{l}{(22, 46)} & \multicolumn{1}{l}{(22, 48)} & \multicolumn{1}{l}{(22, 44)} & \multicolumn{1}{l}{(22, 42)} & \multicolumn{1}{l}{(22, 45)} & \multicolumn{1}{l}{(2, 63)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(1, 68)} & \multicolumn{1}{l}{(0, 44)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(0, 57)} & \multicolumn{1}{l}{(0, 43)} & \multicolumn{1}{l}{(5, 42)} & \multicolumn{1}{l}{(3, 62)} & 47816 \\ 
\textit{\textbf{OPT}} & 50265 & \multicolumn{1}{l}{(0, 61)} & \multicolumn{1}{l}{(0, 61)} & \multicolumn{1}{l}{(13, 48)} & \multicolumn{1}{l}{(16, 51)} & \multicolumn{1}{l}{(11, 40)} & \multicolumn{1}{l}{(1, 57)} & \multicolumn{1}{l}{(1, 59)} & \multicolumn{1}{l}{(1, 68)} & \multicolumn{1}{l}{(1, 67)} & \multicolumn{1}{l}{(1, 69)} & \multicolumn{1}{l}{(1, 65)} & \multicolumn{1}{l}{(1, 63)} & \multicolumn{1}{l}{(1, 66)} & \multicolumn{1}{l}{(0, 65)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(0, 69)} & \multicolumn{1}{l}{(0, 44)} & \multicolumn{1}{l}{(0, 62)} & \multicolumn{1}{l}{(0, 57)} & \multicolumn{1}{l}{(0, 43)} & \multicolumn{1}{l}{(0, 47)} & \multicolumn{1}{l}{(0, 65)} & 49430 \\ \bottomrule
\end{tabular}
}
\caption{Language support of various LLMs for 22 Indian languages and vocab size per language. The first value in each tuple represents the number of language-specific characters, while the second value indicates the count of byte-supported characters.}
\label{tab:llms_details}
\end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering\scriptsize
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|lllllllllllllllllllllll}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{Vocab size} & \multicolumn{23}{c}{Vocab size ( original characters count, byte-supported characters count)} \\ \cline{3-25} 
%  &  & \multicolumn{2}{c|}{Bangla script} & \multicolumn{3}{c|}{Perso-Arbic script} & \multicolumn{8}{c|}{Devanagari} & \multicolumn{10}{c}{Language specific script} \\ \cline{3-25} 
%  &  & \multicolumn{1}{l|}{asm} & \multicolumn{1}{l|}{ban} & \multicolumn{1}{l|}{kas} & \multicolumn{1}{l|}{sin} & \multicolumn{1}{l|}{urd} & \multicolumn{1}{l|}{bod} & \multicolumn{1}{l|}{doi} & \multicolumn{1}{l|}{Hindi} & \multicolumn{1}{l|}{kon} & \multicolumn{1}{l|}{mai} & \multicolumn{1}{l|}{mar} & \multicolumn{1}{l|}{nep} & \multicolumn{1}{l|}{san} & \multicolumn{1}{l|}{guj} & \multicolumn{1}{l|}{kan} & \multicolumn{1}{l|}{mal} & \multicolumn{1}{l|}{mei} & \multicolumn{1}{l|}{odi} & \multicolumn{1}{l|}{pun} & \multicolumn{1}{l|}{sat} & \multicolumn{1}{l|}{tam} & \multicolumn{1}{l|}{tel} & eng \\ \hline
% \textit{\textbf{BLOOM}} & 250680 & \multicolumn{1}{l|}{(59, 2)} & \multicolumn{1}{l|}{(59, 2)} & \multicolumn{1}{l|}{(49, 12)} & \multicolumn{1}{l|}{(48, 19)} & \multicolumn{1}{l|}{(48, 3)} & \multicolumn{1}{l|}{(58, 0)} & \multicolumn{1}{l|}{(59, 1)} & \multicolumn{1}{l|}{(67, 2)} & \multicolumn{1}{l|}{(66, 2)} & \multicolumn{1}{l|}{(67, 3)} & \multicolumn{1}{l|}{(65, 1)} & \multicolumn{1}{l|}{(63, 1)} & \multicolumn{1}{l|}{(65, 2)} & \multicolumn{1}{l|}{(57, 8)} & \multicolumn{1}{l|}{(62, 0)} & \multicolumn{1}{l|}{(66, 3)} & \multicolumn{1}{l|}{(0, 44)} & \multicolumn{1}{l|}{(56, 6)} & \multicolumn{1}{l|}{(55, 2)} & \multicolumn{1}{l|}{(0, 43)} & \multicolumn{1}{l|}{(46, 1)} & \multicolumn{1}{l|}{(61, 4)} & 127581 \\ \hline
% \textit{\textbf{FACLON}} & 65024 & \multicolumn{1}{l|}{(0, 61)} & \multicolumn{1}{l|}{(0, 61)} & \multicolumn{1}{l|}{(12, 49)} & \multicolumn{1}{l|}{(15, 52)} & \multicolumn{1}{l|}{(12, 39)} & \multicolumn{1}{l|}{(2, 56)} & \multicolumn{1}{l|}{(2, 58)} & \multicolumn{1}{l|}{(2, 67)} & \multicolumn{1}{l|}{(2, 66)} & \multicolumn{1}{l|}{(2, 68)} & \multicolumn{1}{l|}{(2, 64)} & \multicolumn{1}{l|}{ (2, 62)} & \multicolumn{1}{l|}{(2, 65)} & \multicolumn{1}{l|}{(0, 65)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(0, 69)} & \multicolumn{1}{l|}{(0, 44)} & \multicolumn{1}{l|}{(0,62)} & \multicolumn{1}{l|}{(0, 57)} & \multicolumn{1}{l|}{(0, 43)} & \multicolumn{1}{l|}{(0, 47)} & \multicolumn{1}{l|}{(0, 65)} & 62278 \\ \hline
% \textit{\textbf{LLAMA-1,2}} & 32024 & \multicolumn{1}{l|}{(23, 38)} & \multicolumn{1}{l|}{(24, 37)} & \multicolumn{1}{l|}{(40, 21)} & \multicolumn{1}{l|}{(45, 22)} & \multicolumn{1}{l|}{(38, 13)} & \multicolumn{1}{l|}{(38, 20)} & \multicolumn{1}{l|}{(38, 22)} & \multicolumn{1}{l|}{(38, 31)} & \multicolumn{1}{l|}{(38, 30)} & \multicolumn{1}{l|}{(38, 32)} & \multicolumn{1}{l|}{(38, 28)} & \multicolumn{1}{l|}{(38, 26)} & \multicolumn{1}{l|}{(38, 29)} & \multicolumn{1}{l|}{(1, 64)} & \multicolumn{1}{l|}{(2, 60)} & \multicolumn{1}{l|}{(33, 36)} & \multicolumn{1}{l|}{(0, 44)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(4, 53)} & \multicolumn{1}{l|}{(0, 43)} & \multicolumn{1}{l|}{(19, 28)} & \multicolumn{1}{l|}{(1, 64)} & 27007 \\ \hline
% \textit{\textbf{MISTRAL}} & 32052 & \multicolumn{1}{l|}{(33, 28)} & \multicolumn{1}{l|}{(34, 27)} & \multicolumn{1}{l|}{(47, 14)} & \multicolumn{1}{l|}{(47, 20)} & \multicolumn{1}{l|}{(45, 6)} & \multicolumn{1}{l|}{(43, 15)} & \multicolumn{1}{l|}{(43, 17)} & \multicolumn{1}{l|}{(43, 26)} & \multicolumn{1}{l|}{(43, 25)} & \multicolumn{1}{l|}{(43, 27)} & \multicolumn{1}{l|}{(43, 23)} & \multicolumn{1}{l|}{(43, 21)} & \multicolumn{1}{l|}{(43, 24)} & \multicolumn{1}{l|}{(5, 60)} & \multicolumn{1}{l|}{(18, 44)} & \multicolumn{1}{l|}{(4, 65)} & \multicolumn{1}{l|}{(0, 44)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(2, 55)} & \multicolumn{1}{l|}{(0, 43)} & \multicolumn{1}{l|}{(22, 25)} & \multicolumn{1}{l|}{(11, 54)} & 27077 \\ \hline
% \textit{\textbf{MPT}} & 50277 & \multicolumn{1}{l|}{(5, 56)} & \multicolumn{1}{l|}{(5, 56)} & \multicolumn{1}{l|}{(31, 30)} & \multicolumn{1}{l|}{(35, 32)} & \multicolumn{1}{l|}{(30, 21)} & \multicolumn{1}{l|}{(22, 36)} & \multicolumn{1}{l|}{(22, 38)} & \multicolumn{1}{l|}{(22, 47)} & \multicolumn{1}{l|}{(22, 46)} & \multicolumn{1}{l|}{(22, 48)} & \multicolumn{1}{l|}{(22, 44)} & \multicolumn{1}{l|}{(22, 42)} & \multicolumn{1}{l|}{(22, 45)} & \multicolumn{1}{l|}{(2, 63)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(1, 68)} & \multicolumn{1}{l|}{(0, 44)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(0, 57)} & \multicolumn{1}{l|}{(0, 43)} & \multicolumn{1}{l|}{(5, 42)} & \multicolumn{1}{l|}{(3, 62)} & 47816 \\ \hline
% \textit{\textbf{OPT}} & 50265 & \multicolumn{1}{l|}{(0, 61)} & \multicolumn{1}{l|}{(0, 61)} & \multicolumn{1}{l|}{(13, 48)} & \multicolumn{1}{l|}{(16, 51)} & \multicolumn{1}{l|}{(11, 40)} & \multicolumn{1}{l|}{(1, 57)} & \multicolumn{1}{l|}{(1, 59)} & \multicolumn{1}{l|}{(1, 68)} & \multicolumn{1}{l|}{(1, 67)} & \multicolumn{1}{l|}{(1, 69)} & \multicolumn{1}{l|}{(1, 65)} & \multicolumn{1}{l|}{(1, 63)} & \multicolumn{1}{l|}{(1, 66)} & \multicolumn{1}{l|}{(0, 65)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(0, 69)} & \multicolumn{1}{l|}{(0, 44)} & \multicolumn{1}{l|}{(0, 62)} & \multicolumn{1}{l|}{(0, 57)} & \multicolumn{1}{l|}{(0, 43)} & \multicolumn{1}{l|}{(0, 47)} & \multicolumn{1}{l|}{(0, 65)} & 49430 \\ \bottomrule
% \end{tabular}
% }
% \caption{Language support of various LLMs for 22 Indian languages and vocab size per language. The first value in each tuple represents the number of language-specific characters, while the second value indicates the count of byte-supported characters.}
% \label{tab:llms_details}
% \end{table*}

